Adaptive Fusion Affinity Graph with Noise-free Online Low-rank Representation for Natural Image Segmentation

Affinity graph-based segmentation methods have become a major trend in computer vision. The performance of these methods relies on the constructed affinity graph, with particular emphasis on the neighborhood topology and pairwise affinities among superpixels. Due to the advantages of assimilating different graphs, a multi-scale fusion graph has a better performance than a single graph with single-scale. However, these methods ignore the noise from images which influences the accuracy of pairwise similarities. Multi-scale combinatorial grouping and graph fusion also generate a higher computational complexity. In this paper, we propose an adaptive fusion affinity graph (AFA-graph) with noise-free low-rank representation in an online manner for natural image segmentation. An input image is first over-segmented into superpixels at different scales and then filtered by the proposed improved kernel density estimation method. Moreover, we select global nodes of these superpixels on the basis of their subspace-preserving presentation, which reveals the feature distribution of superpixels exactly. To reduce time complexity while improving performance, a sparse representation of global nodes based on noise-free online low-rank representation is used to obtain a global graph at each scale. The global graph is finally used to update a local graph which is built upon all superpixels at each scale. Experimental results on the BSD300, BSD500, MSRC, SBD, and PASCAL VOC show the effectiveness of AFA-graph in comparison with state-of-the-art approaches.

==> files/ABSTRACT.tex <==
\begin{abstract}
\setlength{\parindent}{2em}Graph-based segmentation methods have become a major trend in computer vision due to its ability in reflecting global image characters. In this paper, we propose an adaptive fusion framework of graph-based segmentation using subspace clustering. The framework consists of the adjacency graph and a novel adaptive graph, and the two graphs are fused by following a new definition named adaptive node. In the adaptive graph, we first generate a subspace-preserving representation using sparse subspace clustering based on orthogonal matching pursuit, in order to represent supperpixels better. Then, we select adaptive nodes of superpixels according to affinity propagation clustering results. And the adaptive graph is built upon these selected nodes by online low-rank representation. The final result is obtained with partitioning the bipartite graph fused by the adjacency graphs and the adaptive graphs. Experimental results on the Berkeley segmentation database show the superiority of our method in comparison with state-of-the-art methods.
\end{abstract}
%
\begin{keywords}
Graph, image segmentation, superpixels, sparse subspace clustering, online low-rank representation
\end{keywords} 
